A frequency and sensitivity tunable microresonator array for high-speed quantum processor readout

Superconducting microresonators have been successfully utilized as detection elements for a wide variety of applications. With multiplexing factors exceeding 1,000 detectors per transmission line, they are the most scalable low-temperature detector technology demonstrated to date. For high-throughput applications, fewer detectors can be coupled to a single wire but utilize a larger per-detector bandwidth. For all existing designs, fluctuations in fabrication tolerances result in a non-uniform shift in resonance frequency and sensitivity, which ultimately limits the efficiency of band-width utilization. Here we present the design, implementation, and initial characterization of a superconducting microresonator readout integrating two tunable inductances per detector. We demonstrate that these tuning elements provide independent control of both the detector frequency and sensitivity, allowing us to maximize the transmission line bandwidth utilization. Finally we discuss the integration of these detectors in a multilayer fabrication stack for high-speed readout of the D-Wave quantum processor, highlighting the use of control and routing circuitry composed of single flux-quantum loops to minimize the number of control wires at the lowest temperature stage.

==> preamble.tex <==
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage{wasysym,marvosym}
%\usepackage[clean,pdf]{svg}

%\usepackage{bookmark}
\usepackage{epstopdf}
% \epstopdfDeclareGraphicsRule{.svg}{pdf}{.pdf}{%
%  "C:/Program Files/Inkscape/inkscape.exe" -D -z #1 -A \noexpand\OutputFile}
\epstopdfDeclareGraphicsRule{.svg}{pdf}{.pdf}{%
 inkscape.exe -D -z #1 -A \noexpand\OutputFile}
\DeclareGraphicsExtensions{.png,.eps,.pdf,.jpg,.svg}


\RequirePackage{snapshot}

%\usepackage[T1]{fontenc}
\usepackage{amssymb,amsmath}
\usepackage{multirow}
% Or whatever. Note that the encoding and the font should match. If T1
% does not look nice, try deleting the line with the fontenc.
\usepackage{color,colortbl}
\usepackage{xcolor}


\newcommand{\bra}[1]{\ensuremath{\langle#1|}}
\newcommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\newcommand{\braket}[2]{\ensuremath{\langle#1|#2\rangle}}
\newcommand{\ham}{{\mathcal{H}}}
\newcommand{\iqp}{\left|I_q^p\right|}
\newcommand{\Phiqx}{\Phi^x_q}
\newcommand{\Phicjjx}{\Phi^x_{\text{cjj}}}
\newcommand{\Phiccjjx}{\Phi^x_{\text{ccjj}}}
\newcommand{\Philx}{\Phi^x_{L}}
\newcommand{\Phirx}{\Phi^x_{R}}
\newcommand{\Philtx}{\Phi^x_{LT}}
\newcommand{\Phicox}{\Phi^x_{\text{co}}}
\newcommand{\Phiqfpx}{\Phi^x_{\text{qfp}}}
\newcommand{\Philatchx}{\Phi^x_{\text{latch}}}

\newcommand<>{\colorize}[5]{\only<#1>{\textcolor{#3}{#5}}\only<#2>{{\textcolor{#4}{#5}}}}



\definecolor{LRed}{rgb}{1,.8,.8}
\definecolor{MRed}{rgb}{1,.6,.6}
\definecolor{HRed}{rgb}{1,.2,.2}




\graphicspath{
   {Figures//}
   {Figures/SRS-operation//}
   {Figures/NDRO//}
   {Figures/Qubit//}
  % {../TRIUMF/Figures/}
  % {../TRIUMF/Figures/SRS-operation/}
  % {../TRIUMF/Figures/NDRO/}
  % {../TRIUMF/Figures/4-colors/}
  % {../TRIUMF/Figures/fromdenny/}
  % {/net/icebox/home/mwjohnson/Presentation/APS-2013/Figures/}
  % {/net/icebox/home/mwjohnson/Presentation/AQC-2013/}
  % {/net/icebox/home/mwjohnson/Presentation/ASC-2012/Figures/}
  % {../EECE-301/Figures/}
  % {../APS-2013/Figures/}
  % {../AQC-2013/}
  % {../ASC-2012/Figures/}
  % {../EECE-301/Figures/}
}
% beamer specific 

% \AtBeginSubsection[]
% {
%   \begin{frame}
%     \frametitle{Table of Contents}
%     \tableofcontents[currentsection,currentsubsection]
%   \end{frame}
% }

\hypersetup{
    % pdftitle={Your title here},
    % pdfauthor={Your name here},
    % pdfsubject={Your subject here},
    % pdfkeywords={keyword1, keyword2},
  pdfstartpage=1,
    bookmarksnumbered=true,     
    % bookmarksopen=true,         
    bookmarksdepth=5,
    bookmarksopenlevel=5
    %colorlinks=true,            
    % pdfstartview=Fit,           
    % pdfpagemode=UseOutlines,    % this is the option you were lookin for
    % pdfpagelayout=TwoPageRight
}
